Locally-Minimal Probabilistic Explanations

Explainable Artificial Intelligence (XAI) is widely regarding as a cornerstone of trustworthy AI. Unfortunately, most work on XAI offers no guarantees of rigor. In high-stakes domains, e.g. uses of AI that impact humans, the lack of rigor of explanations can have disastrous consequences. Formal abductive explanations offer crucial guarantees of rigor and so are of interest in high-stakes uses of machine learning (ML). One drawback of abductive explanations is explanation size, justified by the cognitive limits of human decision-makers. Probabilistic abductive explanations (PAXps) address this limitation, but their theoretical and practical complexity makes their exact computation most often unrealistic. This paper proposes novel efficient algorithms for the computation of locally-minimal PXAps, which offer high-quality approximations of PXAps in practice. The experimental results demonstrate the practical efficiency of the proposed algorithms.

==> cdefs.tex <==
\definecolor{darkslategray}{rgb}{0.18, 0.31, 0.31} %#2F4F4F
\definecolor{platinum}{rgb}{0.9, 0.89, 0.89} %#E5E4E2
\definecolor{gray}{rgb}{.4,.4,.4}
\definecolor{midgrey}{rgb}{0.5,0.5,0.5}
\definecolor{middarkgrey}{rgb}{0.35,0.35,0.35}
\definecolor{darkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{darkred}{rgb}{0.7,0.1,0.1}
\definecolor{midblue}{rgb}{0.2,0.2,0.7}
\definecolor{darkblue}{rgb}{0.1,0.1,0.5}
\definecolor{darkgreen}{rgb}{0.1,0.5,0.1}
\definecolor{defseagreen}{cmyk}{0.69,0,0.50,0}


==> texfigs/RFs-ffa.tex <==
%
\sisetup{parse-numbers=false,detect-all,mode=text}
\setlength{\tabcolsep}{5pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}


\begin{table}[ht]
\centering
\resizebox{0.99\columnwidth}{!}{
  \begin{tabular}{l>{\lpr}S[table-format=2.0,table-space-text-pre=\lpr]S[table-format=2.0,table-space-text-post=\rpr]<{\rpr}
  S[table-format=2.1]S[table-format=3.2]
  S[table-format=2.1]S[table-format=2]S[table-format=1.2]S[table-format=2.2] }
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (m,~K)}}  & 
\multicolumn{2}{c}{\bf  FFA }  & \multicolumn{4}{c}{\bf  LmFFA}   \\
\cmidrule[0.8pt](lr{.75em}){4-5}
\cmidrule[0.8pt](lr{.75em}){6-9}
  %
& \multicolumn{2}{c}{}  & {\bf Len }  &  {\bf Time}  &  {\bf Len }  & {\bf \% }  & {\bf Prec }  &  {\bf Time }  \\
\toprule[1.2pt]

%
adult  &  12  &  2  &  6.0  &  0.04  &  5.0  &  83  &  0.99  &  0.67 \\
agaricus  &  22  &  2  &  20.0  &  24.66  &  3.4  &  17  &  0.97  &  16.81 \\
compas  &  11  &  2  &  10.0  &  0.37  &  3.9  &  39  &  0.97  &  2.75 \\
german  &  21  &  2  &  21.0  &  155.64  &  3.4  &  16  &  0.97  &  16.01 \\
heart-c  &  13  &  2  &  13.0  &  1.99  &  2.9  &  22  &  0.97  &  2.13 \\
ionosphere  &  34  &  2  &  33.0  &  13.17  &  2.9  &  9  &  0.97  &  14.68 \\
kr\_vs\_kp  &  36  &  2  &  33.0  &  3.58  &  3.3  &  10  &  0.99  &  15.46 \\
lending  &  9  &  2  &  2.0  &  0.03  &  1.7  &  85  &  0.99  &  0.12 \\
mofn\_3\_7\_10  &  10  &  2  &  5.0  &  0.01  &  3.4  &  68  &  0.99  &  0.29 \\
mushroom  &  22  &  2  &  20.0  &  4.72  &  4.3  &  22  &  0.97  &  11.16 \\
parity5+5  &  10  &  2  &  9.0  &  0.03  &  6.7  &  74  &  0.99  &  0.82 \\
recidivism  &  15  &  2  &  15.0  &  0.43  &  5.7  &  38  &  0.97  &  8.49 \\
segmentation  &  19  &  7  &  17.0  &  10.42  &  4.9  &  29  &  0.98  &  4.11 \\
soybean  &  35  &  18  &  34.0  &  230.38  &  8.7  &  26  &  0.97  &  24.36 \\
tic\_tac\_toe  &  9  &  2  &  9.0  &  0.03  &  3.4  &  38  &  0.97  &  2.17 \\
twonorm  &  20  &  2  &  15.0  &  0.04  &  8.1  &  54  &  0.98  &  1.97 \\
vote  &  16  &  2  &  16.0  &  1.26  &  2.5  &  16  &  0.98  &  10.65 \\
%

\bottomrule[1.2pt]
\end{tabular}
}
\caption{%
\footnotesize{
  Detailed performance evaluation of computing LmFFA for RFs.
%
%The table shows results for 17 datasets containing binary and 
%categorical data. The maximum tolerance  was fixed to 0.05, i.e.\ 
%$\Tau = 0.95$.
%%
%Columns {\bf m} and {\bf K} report, respectively, the
%number of features and classes in the dataset.
%%
%Columns {\bf Len} and  {\bf Time}  report, resp., the average length 
%of computed FFA's (resp.\ LmFFA) and  the average runtime for computing 
%such explanations.
%%
%Column {\bf Prec} reports the average precision of the probabilistic explanations.
}}
\label{tab:RFs-ffa}
\end{table}



==> texfigs/RFs-sat.tex <==
%
\sisetup{parse-numbers=false,detect-all,mode=text}
\setlength{\tabcolsep}{5pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}


\begin{table}[ht]
\centering
\resizebox{0.99\columnwidth}{!}{
  \begin{tabular}{l>{\lpr}S[table-format=2.0,table-space-text-pre=\lpr]S[table-format=2.0,table-space-text-post=\rpr]<{\rpr}
  S[table-format=2.1]S[table-format=2.2]
  S[table-format=2.1]S[table-format=2]S[table-format=1.2]S[table-format=2.2] }
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (m,~K)}}  & 
\multicolumn{2}{c}{\bf  AXp }  & \multicolumn{4}{c}{\bf  LmPAXp}   \\
\cmidrule[0.8pt](lr{.75em}){4-5}
\cmidrule[0.8pt](lr{.75em}){6-9}
  %
& \multicolumn{2}{c}{}  & {\bf Len }  &  {\bf Time}  &  {\bf Len }  & {\bf \% }  & {\bf Prec }  &  {\bf Time }  \\
\toprule[1.2pt]

%
adult  &  12  &  2  &  5.6  &  0.19  &  3.2  &  57  &  0.97  &  0.99 \\
agaricus  &  22  &  2  &  10.0  &  0.06  &  3.3  &  33  &  0.96  &  3.78 \\
compas  &  11  &  2  &  5.6  &  0.12  &  3.6  &  64  &  0.97  &  0.77 \\
german  &  21  &  2  &  12.3  &  0.36  &  3.2  &  26  &  0.97  &  5.40 \\
heart-c  &  13  &  2  &  5.5  &  0.07  &  3.0  &  55  &  0.97  &  0.39 \\
ionosphere  &  34  &  2  &  21.5  &  0.06  &  2.9  &  13  &  0.96  &  6.59 \\
kr\_vs\_kp  &  36  &  2  &  8.1  &  0.08  &  3.5  &  43  &  0.98  &  0.84 \\
lending  &  9  &  2  &  2.2  &  0.10  &  1.7  &  77  &  0.99  &  0.15 \\
mofn\_3\_7\_10  &  10  &  2  &  3.1  &  0.06  &  2.8  &  90  &  0.99  &  0.13 \\
mushroom  &  22  &  2  &  9.2  &  0.07  &  4.2  &  46  &  0.97  &  2.30 \\
parity5+5  &  10  &  2  &  6.8  &  0.23  &  6.4  &  94  &  0.99  &  0.38 \\
recidivism  &  15  &  2  &  7.9  &  0.48  &  5.8  &  73  &  0.97  &  1.75 \\
segmentation  &  19  &  7  &  8.1  &  0.39  &  4.9  &  60  &  0.98  &  0.76 \\
soybean  &  35  &  18  &  15.6  &  2.05  &  8.9  &  57  &  0.97  &  4.07 \\
tic\_tac\_toe  &  9  &  2  &  5.0  &  0.09  &  3.3  &  66  &  0.97  &  0.58 \\
twonorm  &  20  &  2  &  10.4  &  0.05  &  4.4  &  42  &  0.97  &  1.35 \\
vote  &  16  &  2  &  5.6  &  0.07  &  2.6  &  46  &  0.98  &  1.16 \\
%

\bottomrule[1.2pt]
\end{tabular}
}
\caption{%
\footnotesize{
  Detailed performance evaluation of computing LmPAXp for RFs.
%
The table shows results for 17 datasets containing binary and 
categorical data. The maximum tolerance  was fixed to 0.05, i.e.\ 
$\Tau = 0.95$.
%
Columns {\bf m} and {\bf K} report, respectively, the
number of features and classes in the dataset.
%
Columns {\bf Len} and  {\bf Time}  report, resp., the average length 
of computed AXp's (resp.\ LmPAXp) and  the average runtime for computing 
such explanations.
%
Column {\bf Prec} reports the average precision of the probabilistic explanations.
}}
\label{tab:RFs-sat}
\end{table}


